Integrating Additional Knowledge Into Estimation of Graphical Models

In applications of graphical models, we typically have more information than just the samples themselves. A prime example is the estimation of brain connectivity networks based on fMRI data, where in addition to the samples themselves, the spatial positions of the measurements are readily available. With particular regard for this application, we are thus interested in ways to incorporate additional knowledge most effectively into graph estimation. Our approach to this is to make neighborhood selection receptive to additional knowledge by strengthening the role of the tuning parameters. We demonstrate that this concept (i) can improve reproducibility, (ii) is computationally convenient and efficient, and (iii) carries a lucid Bayesian interpretation. We specifically show that the approach provides effective estimations of brain connectivity graphs from fMRI data. However, providing a general scheme for the inclusion of additional knowledge, our concept is expected to have applications in a wide range of domains.

==> Otherways.tex <==
 \subsection{Other ways to include \addinfo}
There are other studies aimed at incorporating \addinfo\ into graphical models, we mention two representative examples. The first one, proposed by Fang Han, adds pairwise penalty terms into the regressions of neighborhood selection
\begin{equation*}
\hat\beta^{j,r,\gamma}\in\underset{\substack{\beta\in \mathbb R^p\\\beta_j=0}}
{\operatorname{arg min}}\big\{\normtwo{X^j-X\beta}^2+ r\normone{\beta}+ \gamma\underset{\substack{\mathcal G_{\textbf L}\\k_1\,\sim\, k_2}}{\sum}\ |\beta_{k_1}-\beta_{k_2}| \big\}\,,
 \label{pair penalty} 
 \end{equation*} 
where $r, \gamma\in \mathbb R$ are tuning parameters, $\textbf L$ is the 3-D locations of the nodes equipped with a certain metric $\rho$, and $\mathcal G_{\textbf L}$ is the geodesic graph corresponding to $\textbf L$, with different structures inducing different graphs. 
The second one stated in~\cite{Harezlak} operates under the framework of generalized singular value decomposition. The general formulation is the sum of a squared-error loss with quadratic penalty
\begin{equation*}
\hat\beta^{\lambda,L}\in\underset{\beta} 
{\operatorname{arg min}}
\big\{\normtwo{\textbf{y} -X\beta}^2 + \lambda\norm{L\beta}^2_{L^2} \big\}\,,
 \label{second other} 
 \end{equation*} 
where $L$ is an $m \times p$ discretized penalty operator. 

In comparison to these two methods, our proposed method has a direct Bayesian interpretation of the incorporated structural information, and is more convenient to optimize using existing lasso packages. Moreover, in contrast to the first approach discussed above, we have to calibrate only one tuning parameter, which is better understood and easier to compute than calibrating several tuning parameters.

